Combining Symbolic Execution and Model Checking to Verify MPI Programs

Message passing is the standard paradigm of programming in high-performance computing. However, verifying Message Passing Interface (MPI) programs is challenging, due to the complex program features (such as non-determinism and non-blocking operations). In this work, we present MPI symbolic verifier (MPI-SV), the first symbolic execution based tool for automatically verifying MPI programs with non-blocking operations. MPI-SV combines symbolic execution and model checking in a synergistic way to tackle the challenges in MPI program verification. The synergy improves the scalability and enlarges the scope of verifiable properties. We have implemented MPI-SV (footnote: https://mpi-sv.github.io) and evaluated it with 111 real-world MPI verification tasks. The pure symbolic execution-based technique successfully verifies 61 out of the 111 tasks (55\%) within one hour, while in comparison, MPI-SV verifies 100 tasks (90\%). On average, compared with pure symbolic execution, MPI-SV achieves 19x speedups on verifying the satisfaction of the critical property and 5x speedups on finding violations.

==> sec8.tex <==
%!TEX root = main.tex

\appendix

\section{Appendix}

\subsection{Proof of Theorem \ref{thm:independence}}

\textbf{Theorem 3.1} Given an action $a\in\{issue(o),B,W,SR\}$ and action $b$, for $S\in \mathcal{G}$, if $a, b\in enabled(S)$, then $(a,b)\in\mathcal{I}$.

\begin{proof}


\textbf{Case 1: $a=issue(o)$.}\quad When $a=issue(o)$ and $a,b\in enabled(S)$, $b$ can be $issue(o')$, $W$, $SR$, or $SR^*$ \wrt the transition rules.

$(1)\ b=issue(o').$\quad Suppose $rank(o){=}i$, $rank(o'){=}j$, and $i{\neq} j$. Since issue action can only block its process, $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$. In addition, $a(b(S)){=}b(a(S)){=}(\dots,s_i[update(\mathcal{F},o),$\\$Stat{:=}Stat', \mathcal{B}.push(o)],\!\dots,s_j[update(\mathcal{F},o'),Stat{:=}Stat',\mathcal{B}.push(o')],\!\dots)$. Hence, $(a,b)\in\mathcal{I}$.

$(2)\ b=W.$\quad
Suppose $rank(o){=}i$, $rank_a(W){=}j$, and $i\neq j$. Since $issue(o)$ can only block $\textsf{Proc}_i$ and $W$ can only make $\textsf{Proc}_j$ active, $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$. In addition, $a(b(S)){=}b(a(S)){=}$\\$( \dots,s_i[update(\mathcal{F},o), Stat{:=}Stat', \mathcal{B}.push(o)],\dots,s_j[update(\mathcal{F},\verb"Wait"),\mathcal{B}.pull(\verb"Wait")],\dots)$. Hence, $(a,b){\in}\mathcal{I}$.

$(3)\ b{=}SR{\lor} b{=}SR^*.$\quad Suppose $b{=}(p,q)$, $rank(o){=}i$, $rank(p){=}j_1$, and $rank(q){=}j_2$. For $i{\neq} j_1{\land} i{\neq} j_2$: since $issue(o)$ only updates the state of $\textsf{Proc}_i$, $ready(p,s_{j_1})$ and $ready(q,s_{j_2})$ will not be affected. On the other hand, executing $(p,q)$ cannot make $\textsf{Proc}_i$ blocked. Hence $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$.
$a(b(S)){=}b(a(S)){=}( \dots,s_i[update(\mathcal{F},o),Stat{:=}Stat',\mathcal{B}.push(o)],\dots,s_{j_1}[update(\mathcal{F},p), \mathcal{B}.pull(p)],$\\$\dots,s_{j_2}[update(\mathcal{F},q),\mathcal{B}.pull(q)],\dots)$. For
$i{=}j_1$: since $issue(o)$ and $b$ are co-enabled, $index(o){>}index(p)$ and $p$ is non-blocking. Due to $index(o){>}index(p)$, $issue(o)$ has no effect on $ready(p,s_{j_1})$. On the other hand, since $p$ is non-blocking, executing $(p,q)$ cannot make $\textsf{Proc}_i$ blocked. Hence $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$. $a(b(S)){=}b(a(S)){=}(\dots,s_i[update(\mathcal{F},o),Stat{:=}Stat', \mathcal{B}.pull(p),\mathcal{B}.push(o)],\dots,$\\$s_{j_2}[update(\mathcal{F},q),\mathcal{B}.pull(q)],\dots)$. For $i{=}j_2$, the proof is similar. Hence $(a,b){\in}\mathcal{I}$.

\textbf{Case 2: $a{=}B$.}\quad When $a{=}B$ and $a,b{\in} enabled(S)$, $b$ can be $(p,q){\in}\{SR,SR^*\}$, where both $p$ and $q$ are non-blocking operations. Suppose $rank(p){=}i$ and $rank(q){=}j$, executing $(p,q)$ does not affect $B{\in} s_i.\mathcal{B}$ and $B{\in} s_j.\mathcal{B}$. On the other hand, executing $B$ only pulls \verb"Barrier" from $s_i.\mathcal{B}$ and $s_j.\mathcal{B}$, which has no effect on $ready(p,s_i)$ and $ready(q,s_j)$.
So $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$. Compared with all the other local states, in addition to updating process status and removing $\verb"Barrier"$ from the buffer of each process, $s_i$ and $s_j$ remove $p$ and $q$ from the buffer, respectively. $a(b(S)){=}b(a(S)){=}(s_0[update(\mathcal{F},\verb"Barrier"),\mathcal{B}.pull(\verb"Barrier")],\dots,s_i[update(\mathcal{F},\verb"Barrier"),$\\$\mathcal{B}.pull(\verb"Barrier"),\mathcal{B}.pull(p)],\dots,s_j[update(\mathcal{F},\verb"Barrier"),\mathcal{B}.pull(\verb"Barrier"),\mathcal{B}.pull(q)],\dots,$\\$
s_n[update(\mathcal{F},\verb"Barrier"),\mathcal{B}.pull(\verb"Barrier")])$.  Hence, $(a,b){\in}\mathcal{I}$.

\textbf{Case 3: $a{=}W$.}\quad When $a{=}W$ and $a,b{\in} enabled(S)$, $b$ can be $issue(o)$, $W$, and $(p,q){\in}\{SR,SR^*\}$. Since $\mathcal{I}$ is symmetric and $(issue(o),W)\in\mathcal{I}$, $(W,issue(o)){\in}\mathcal{I}$.

$(1)\ b{=}W.$\quad Suppose $a{=}\verb"Wait"(r_1)$, $b{=}\verb"Wait"(r_2)$, $rank_a(a){=}i$, and $rank_a(b){=}j$ ($i{\neq} j$).
Executing $\verb"Wait"(r_1)$ or $\verb"Wait"(r_2)$ cannot affect $ready(\verb"Wait"(r_2),s_j)$ or $ready(\verb"Wait"(r_1),s_i)$, so $b{\in} enabled(a(S))$ and also $a{\in} enabled(b(S))$. $a(b(S)){=}b(a(S)){=}(\dots,s_i[update(\mathcal{F},\verb"Wait"(r_1)),\mathcal{B}.pull(\verb"Wait"(r_1))],\dots,s_j[update(\mathcal{F},$\\$\verb"Wait"(r_2)),\mathcal{B}.pull(\verb"Wait"(r_2))],\dots)$. Hence, $(a,b){\in}\mathcal{I}$.

$(2)\ b{=}SR{\lor} b{=}SR^*.$\quad
Suppose $b{=}(p,q)$, $rank_a(W){=}i$, $rank(p){=}j_1$ and $rank(q){=}j_2$. For $i{\neq} j_1{\land} i{\neq} j_2$: executing $\verb"Wait"$ has no effect on $ready(p,s_{j_1})$ and
$ready(q,s_{j_2})$. On the other hand, executing $(p,q)$ does not affect $ready(\verb"Wait",s_i)$. So $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$. $a(b(S)){=}b(a(S)){=}(\dots $\\$s_i[update(\mathcal{F},\verb"Wait"),\mathcal{B}.pull(\verb"Wait")],\dots,s_{j_1}[update(\mathcal{F},p),\mathcal{B}.pull(p)],\dots,s_{j_2}[update(\mathcal{F},q),$\\$\mathcal{B}.pull(q)],\dots)$.
For $i{=}j_1$: $p$ is non-blocking and $index(W){>}index(p)$.
Clearly, executing $\verb"Wait"$ has no effect on $ready(p,s_{j_1})$. Besides,  $ready(q,s_{j_2})$ and $ready(\verb"Wait",s_i)$ are not affected by executing $(p,q)$.
So $b{\in} enabled(a(S))$ and $a{\in} enabled(b(S))$.
$a(b(S)){=}b(a(S)){=}(\dots ,s_i[update(\mathcal{F},\verb"Wait"),\mathcal{B}.pull(p),$\\$\mathcal{B}.pull(\verb"Wait")]\dots,s_{j_2}[update(\mathcal{F},q),\mathcal{B}.pull(q)],\dots)$. The proof for $i{=}j_2$ is similar. Hence, $(a,b){\in}\mathcal{I}$.

\textbf{Case 4: $a{=}SR$.}\quad When $a{=}SR$ and $a,b{\in} enabled(S)$, $b$ can be $issue(o)$, $B$, $W$, and $(p,q){\in}\{SR,SR^*\}$. Since $\mathcal{I}$ is symmetric and $(issue(o),SR), (B,SR), (W,SR){\in}\mathcal{I}$, $(SR,issue(o)),(SR,B),(SR,W){\in}\mathcal{I}$.

$b{=}SR{\lor} b{=}SR^*$.\quad
Suppose $a{=}(p_1,p_2)$ and $b{=}(q_1,q_2)$. Executing $SR/SR^*$ pulls the corresponding operations from the buffer. The co-enableness of $a$ and $b$ ensures that the pulled action is not in the match pair of the other. So $b{\in} enabled(a(S){\land} a{\in} enabled(b(S))$.
If $\forall\,i,j{\in}\{1,2\},\ rank(p_i){\neq} rank(q_j)$, changing the order of updating the statuses of different processes is insensitive to the resulting state. Once $\exists\,i,j{\in}\{1,2\},\ rank(p_i){=}rank(q_j)$, suppose $index(p_i){<}index(q_j)$, then $p_i$ must be non-blocking. Similar to the second case ($i {=} j_1$) when $a {=} W \wedge (b {=} SR {\vee} b {=} SR^*)$ (\cf \textbf{Case 3}), changing the order of $update(\mathcal{F},p_i)$ and $update(\mathcal{F},q_j)$ cannot change the resulting state.
On the other hand, whatever the relationship of $rank(p_i)$ and $rank(q_j)$ is, changing the order of buffer pulling operations makes no difference for the resulting state. So $a(b(S)){=}b(a(S))$. Hence $(a,b){\in}\mathcal{I}$.

In conclusion, the theorem holds.
\end{proof}

